L*ReLU: Piece-wise Linear Activation Functions for Deep Fine-grained Visual Categorization

Deep neural networks paved the way for significant improvements in image visual categorization during the last years. However, even though the tasks are highly varying, differing in complexity and difficulty, existing solutions mostly build on the same architectural decisions. This also applies to the selection of activation functions (AFs), where most approaches build on Rectified Linear Units (ReLUs). In this paper, however, we show that the choice of a proper AF has a significant impact on the classification accuracy, in particular, if fine, subtle details are of relevance. Therefore, we propose to model the degree of absence and the presence of features via the AF by using piece-wise linear functions, which we refer to as L*ReLU. In this way, we can ensure the required properties, while still inheriting the benefits in terms of computational efficiency from ReLUs. We demonstrate our approach for the task of Fine-grained Visual Categorization (FGVC), running experiments on seven different benchmark datasets. The results do not only demonstrate superior results but also that for different tasks, having different characteristics, different AFs are selected.

==> sections/experiments_tmp.tex <==
\section{Results}

%Animal images of Image Net dataset classify into following categories:\\
%1-Mammals\\
%2-Birds\\
%3-Reptiles\\
%4-Amphibians\\
%5-Fish\\

\iffalse

\begin{table}[h!]
 % title of Table
\centering % used for centering table
\begin{center}
\begin{tabular}{l|*{6}{c}|r}\hline	
Dataets  & Elish & Swish & Relu  \\
\hline\\
ImageNet Dataset & 71.89\% & 69.46\% & 68.99\%  \\ \hline\\
Fashion Image Dataset  & 53.61\% & 51.52\% & 51.59\%   \\ \hline\\
\hline
\end{tabular}
\label{table:taskb} % is used to refer this table in the text
\end{center}
\caption{Results of Super Class learning }
\end{table}

Images of Fashion image dataset classify based on their brands like Gucci, Dior
\\
\fi


Results for Fine-grained Dataset as follows:\\

\begin{table}[!h]
\centering
\begin{center}
\begin{tabular}{l|*{6}{c}|r}\hline	
Dataset & ELU & Swish & ReLU & Leaky ReLU (best slop)  \\
\hline\\
Stanford Dogs Dataset    & 35.6 \% & 37.13\% & 36.37\% & 37.62\% \\
\hline\\
Caltech-UCSD Birds 200   & 38.21\% & 38.53\% & 38.38\% & 44.45\% \\
\hline\\
Car stanford Dataset     & 41.92\% & 45.49\% & 36.02\% & 46.97\% \\
\hline
iFood Dataset            & 37.69\% & 40.78\% & 37.53\% & 43.09\% \\
\hline
\\\hline
\end{tabular}
\label{table:taskb}
\end{center}
\caption{Results  of Fine-grained Dataset classification}
\end{table}


\begin{figure}[!ht]
\centering
\begin{subfigure}{0.45\textwidth}
	\centering
	\includegraphics[width=\textwidth]{results/dog_loss_allslops_test.png}
	\caption{Dog Dataset}
	\label{fig:loss:a}		
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
	\centering
	\includegraphics[width=\textwidth]{results/bird_loss_allfunctions.png}
	\caption{Bird Dataset}
	\label{fig:loss:b}		
\end{subfigure}

\begin{subfigure}{0.45\textwidth}
	\centering
	\includegraphics[width=\textwidth]{results/dog_loss_allfunctions_train.png}
	\caption{ Loss values for training}
	\label{fig:loss:c}		
\end{subfigure}
\label{fig:loss}		
\end{figure}

\prmk{Are there (already) other loss curves to be shown here? How much effot is it to generate them? This should be something which can be done just in a few minutes}


==> sections/experiments_trash.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}{0.45\textwidth}
	\centering
	 \includegraphics[width=\textwidth,height=5cm]{results/cifar10_acc_plot.pdf}
	\caption{CIFAR-10}
	\label{fig:slope:e}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
	\centering
	 \includegraphics[width=\textwidth,height=5cm]{results/cifar100_acc_plot.pdf}
	\caption{CIFAR-100}
	\label{fig:slope:f}
\end{subfigure}
\caption{Classification accuracy vs. slope evaluated on the CIFAR datatsets.}
\label{fig:cifar-slopes}
\end{figure}


\begin{figure}[!ht]
\centering
\begin{subfigure}{0.2\textwidth}
	\centering
	\includegraphics[page=1, width=\textwidth]{results/Tizit_plot_BMVC.pdf}
	\caption{Bird-UCSD}
	\label{fig:slope:a}		
\end{subfigure}%
\begin{subfigure}{0.2\textwidth}
	\centering
	\includegraphics[page=2, width=\textwidth]{results/Tizit_plot_BMVC.pdf}
	\caption{Car Stanford}
	\label{fig:slope:b}
\end{subfigure}%
\begin{subfigure}{0.2\textwidth}
	\centering
     \includegraphics[page=3, width=\textwidth]{results/Tizit_plot_BMVC.pdf}
	\caption{Dog Stanford}
	\label{fig:slope:c}
\end{subfigure}%
\begin{subfigure}{0.2\textwidth}
	\centering
	 \includegraphics[page=4, width=\textwidth]{results/Tizit_plot_BMVC.pdf}
	\caption{iFood}
	\label{fig:slope:d}
\end{subfigure}%
\begin{subfigure}{0.2\textwidth}
	\centering
	 \includegraphics[page=5, width=\textwidth]{results/Tizit_plot_BMVC.pdf}
	\caption{Aircraft}
	\label{fig:slope:d}
\end{subfigure}
\caption{ Accuracy vs. slope for fine-grained datasets}
\label{fig:slopeall}
\end{figure}


%%%%%Loss_plot_test************
centering
	\begin{subfigure}{0.45\textwidth}
    	\centering
    	\includegraphics[page=1, width=\textwidth]{results/Loss_Result.pdf}
    	\caption{Aircraft Dataset}
    %	\caption{Coarse-grained datasets: mean and standard deviation for all datasets and AFs.}
	\end{subfigure}%
	\begin{subfigure}{0.45\textwidth}
    	\centering
    	\includegraphics[page=2, width=\textwidth]{results/Loss_Result.pdf}
    	\caption{Car Dataset}
        %	\caption{Coarse-grained datasets: mean and standard deviation for all datasets and AFs.}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.45\textwidth}
        	\centering
        	\includegraphics[page=3, width=\textwidth]{results/Loss_Result.pdf}
        	\caption{Dog Dataset}
            %	\caption{Coarse-grained datasets: mean and standard deviation for all datasets and AFs.}
	\end{subfigure}%
	\begin{subfigure}{0.45\textwidth}
    	\centering
    	\includegraphics[page=4, width=\textwidth]{results/Loss_Result.pdf}
    	\caption{Bird Dataset}
        %	\caption{Coarse-grained datasets: mean and standard deviation for all datasets and AFs.}
	\end{subfigure}%
	\hfill
    	\begin{subfigure}{0.45\textwidth}
        	\centering
        	\includegraphics[page=5, width=\textwidth]{results/Loss_Result.pdf}
        	\caption{Food Dataset}
            %	\caption{Coarse-grained datasets: mean and standard deviation for all datasets and AFs.}
    	\end{subfigure}%
    	\hfill

==> sections/introduction_190426.tex <==
\section{Introduction}


Image processing is dominating the modern lifestyle. From its safety critical aspect to entertainment aspects. Safety-critical aspects can be included image processing methods for Bio-metric applications. They aimed at providing autonomous control and security.
%control access to mobile devices, to reduce fraudulent transactions in electronic commerce, and even to prevent illegal immigration.
Bio-metric consists of object detection and classification.  Image classification means assigns a label to an image or an object. It is divided into two sub-categories; Coarse-grained visual classification (CGVC) and Fine-grained visual classification (FGVC).
Different from CGVC that aims to distinguish basic-level categories, FGVC deal with distinguishing objects that belong to the same basic category, but not the same class such as animal species, man-made objects like car models. The high visual similarly between class makes FGCV super challenging task.

On the other hand, recent developments in deep neural network drastically increase the performance of CGVC tasks. To this purpose, the impact of initialization, Batch-normalization, network architecture, hyperparameter optimization, data augmentation, and most important one's activation function are well studied. Many of these studies have been extended to FGVC. For example; trainable deep features on CGVC like ImageNet are transferred to FGVC. Moreover, Convolutions Neural Networks(CNNs) improves FGVC by learning discriminative features.
Basic CNNs can only
achieve the moderate performance, because it is relatively
difficult for them to focus on the subtle differences of object's parts without special design. Therefore,
\cite{mb:sanchez11,mb:perronnin15}  part local information is merged into CNNs to represent the deep features of object parts. Image resolution and data augmentation are also investigated by [].

A broader class of activation functions, namely the rectified unit family is considered as a key   success in modern deep neural network[], in particular for CGVC.
However, no one studies the role of activation function especially rectify  unit family in FGVC which is the overall purpose of this paper.


In our paper[], we showed that  generating an optimal activation function is very task specific and for different task different shape of the activation function is meaningful. In this paper, we define the shape of the activation function in terms of the feature's absence and feature's presence. When a feature is present in the current sample, an activation function assigns value>0 to signal to show how strongly a feature is present.  The other way around, the feature's absence means a detected feature is not present in the current sample. For example, when all feature's absence are mapping to zero, activation function looks like ReLU. 

Concerning FGVC,  we found that both feature 's absence and presence are meaningful.A part from the shape of the activation function. The scale (slop) of the activation function is also important as we discuss in the section' Discussion.'


DNN
\cite{pr:goodfellow16,pr:lecun15} have recently become popular and are now successfully applied for a wide range of applications. However, since increasingly more complex and deeper networks are of interest, strategies are required to make neural network training efficient and stable.

While initialization (e.g., \cite{pr:sutskever13,pr:mishkin15}) 
and normalization techniques (e.g., \cite{pr:laurent16}) are well studied, a relevant and important factor is often neglected: the role of AFs.






Fine-Grained Visual Classification (FGVC) aims to differentiate between 
hard-to-distinguish object classes, ranging from species of birds to man-made objects like models of cars. What makes FGCV datasets different from coarse-grained visual classification (CGVC) is   significant visual similarity among samples.  FGVC involves in subtle visual differences between classes and often exhibits long tails in the data distribution. As a second challenge, FGVC tasks always lack in training data since domain knowledge is required for data acquisition. These problems makes FGVC challenging even for state of the art approaches. To address these challenges, FGVC systems should possess two main characteristics: (1) sufficient discriminative capability to distinguish the subtle differences among the subcategories, and (2) strong learning power to explore similarities among categories.

So far, many approaches have been proposed to provide such characteristics but no one viewing FGVC problem through the lens of activation function. Strickly Speaking, it shown in this paper, providing  a proper activation function in terms of shape and slop of function significantly improve FGVC performance. Most popular activation functions such as \relu, \elu are contractive mapping which is not a proper characteristic for FGVC. Because this mapping is less sensitive to changes in input values and as it is mentioned before subtle changes and differences are meaningful for FGCV. Therefore, we need activation functions which are less contractive like \func{Leaky ReLU} with an appropriate Lipchitz constant (slop).



The rest of the paper is organized as follows: First, in Sec.~\ref{sec:related}, we discuss the related work in context of activation functions and existing approaches for fine-grained image classification. Next, in Sec.~\ref{sec:nipcaf}, we introduce Negative Information Preserving Contractive Activation Functions (NIPCAFs) and discuss why these are of importance for the problem on hand. Then, these findings are discussed based on experimental results in Sec.~\ref{sec:experiments}. Finally, we conclude our work and give an outlook on future work in Sec.~\ref{sec:conclusion}.






==> sections/introduction_mina.tex <==
% rmkp: As the information is quite redundant to Sec.4 and many points are too technical for an introduction (=reads like a method's section, I will take the relevant parts and move them to Sec.4. Moreover, we cannot leave out the FG problem in the introduction ...


\section{Introduction}

Deep Convolutional Neural Networks (\eg, \cite{pr:goodfellow16,pr:lecun15} have recently shown to be very beneficial for a variety of applications in the field of Computer Vision. Thus, there has been, for instance, a considerable interest in designing new network architectures, introducing efficient data augmentation techniques, and improving the parameter optimization. In addition, to increase the robustness and the speed of training also different techniques for initialization (e.g., \cite{pr:sutskever13,pr:mishkin15}) and normalization (e.g., \cite{pr:laurent16}) have been explored. However, one relevant and important parameter is mostly ignored, the proper choice of the non-linear activation function (AF). 

In fact, recent works have demonstrated that introducing \cite{pr:klambauer17,pr:clevert16,pr:elfwing18,pr:glorot11,pr:gulcehre16}) and learning \cite{pr:ramachandran18,pr:basirat19,pr:hayou18,pr:li18a} new AFs and their parameters are beneficial in terms of convergence speed and training stability, however, also that only minor improvements for the final tasks can be achieved. Thus, most deep learning approaches use Rectified Linear Units (\relu) \cite{pr:nair10}, which have proven to be reliable and allow for fast learning. In contrast, we are able to show that the proper choice of the AF can significantly improve the performance of deep neural networks for practical applications. 

Recent studies, further clarified the importance of activation functions in deep neural networks by introducing concepts like degrees of presence and absence \cite{pr:clevert16}. A feature's presence or absence in the current sample set is exposed by the returned value of an AF. More specifically, if a feature is present in the current sample set, an activation function is supposed to return a value greater than zero; on the other hand, if a feature is absent it returns a value smaller or equal to zero. Informally speaking, an AF is a mapping function $f: X \to Y$.
The values in the domain $X$ are features from which the neural network learns.
In the sense of a mapping function, an effective $f$ is usually a nonlinear transformation from features $X$ to the range $Y$ that represents to which extent the features are present or absent.

Most commonly used activation functions to this date have bounded first derivatives, which makes them Lipschitz continuous mappings.
A Lipschitz continuous function is a strong form of uniform continuity for functions. 
Intuitively, a Lipschitz continuous function is limited in how fast it can change \cite{sohrab2003}.
That is, there exists a real number such that, for every pair of points on the graph of this function, the absolute value of the slope of the line connecting them is not greater than this real number; we call the smallest such bound the Lipschitz constant of the function (or modulus of uniform continuity) \cite{sohrab2003}.
Given a Lipschitz function, if its Lipschitz constant is greater than $1$ we call it an `expansive map', otherwise a `contractive map'. 

It is shown that feature's absence and presence are vital to both the performance and the robustness of neural networks. Knowing above concept, in this paper, we show how an AF with proper Lipschitz constant fine tunes this aspect of neural networks.
The first step to better understand the gist of our discussion is to digest the following rewriting rule for AFs:
\[
f(x)= p(x\geq 0) + n(x < 0)
\]
where sub-function $p$ is defined as:
\[
p(x) = \max(\phi(x),0)
\]
and sub-function $n$ is defined as:
\[
n(x) = \min(\eta(x),0)
\]
Meanwhile $p: X \to Y$ transforms positive $x \in X$ to either positive $y \in Y$ or $0$.
Similarly, $n: X \to Y$ ensures all negative $x \in X$ are either mapped to negative $y \in Y$ or $0$. 
It is easy to see, we can rewrite almost all popular AFs to this date in above form.
Please note that rewriting a Lipschitz continuous AF in above form preserves Lipschitz continuity for both $n(x)$ and $p(x)$.
Having distinguished the pieces of an AF that resides in the first and third quadrants of a Cartesian system, we are now able to discuss how to fine tune feature's degree of presence and absence by tweaking Lipschitz constant of $p(x)$ and $n(x)$, respectively.
For example, $ReLU(x)=\max(x,0)$ maps the presence of the features via identity with Lipschitz constant $1$, whereas all missing features are mapped to zero with Lipschitz constant $0$ dying all information about feature's absence.




==> sections/old_abstract.tex <==
Deep convolutional neural networks paved the way for significant improvements in image classification during the last years. However, even though the complexity/difficulty and the specific charactericits of the tasks are highly varying, mostly the same existing architectures are used and just slightly adopted. This, in particular, applies to the selection of activation functions, where most approaches build on Rectified Linear Units (ReLUs). In this paper, however, we show that the selection of a proper activation function has a significant impact on the classification accuracy. For this purpose, we study the problem of Fine-grained Visual Classification (FGVC), where in contrast to Coarse-grained Visual Classification (CGVC) even tiniest details are of relevance for successful classification. To preserve the most valuable information to robustly discriminate between very similar samples, the contractive properties of the selected activation function (AF) play a crucial role. This can be analyzed by studying the Lipschitz-constant of a function, which is a non-trivial task. Thus, we introduce a linear approximation of such functions  similar to ReLU: Lipschitz ReLU (LiReLU). The experimental evaluation on seven different datasets shows not only an improvement of up to $10\%$, but also that for different tasks different Lipschittz-levels are required.


==> sections/open_questions.tex <==
\prmk{General comments, also taking into account those of R3:
\\
\\
* Maybe we could also include other CG datasets, showing the same results as CIFAR?
\\
\\
* It would be easy to also include SELU. Are there are any other (parametric) function which can be easily included?
\\
\\
* Initialization would have some impact, but we would not take this into account as this would be out-of-scope?
\\
\\
* Why was the cropped VGG used? How much effort would it be to apply the whole thing also for different architectures?
\\
\\
* Since we have more space now, all other training parameters such as number of epochs, learning rate, etc. should be given!
\\
\\
* Doing the same thing with the positive part would be of course of interest. However, in this case we would run into never ending parameter combinations? But fixing the best slope for the negative part, this could be worth a try?
\\
\\
* The proposed "held-out" validation would be also worth giving it a try. Maybe, we could do the same thing as for the GA? Running the training on a rather shallow architecture and then to apply the "learned" parameters for deeper ones?
\\
\\
* Using different ks would be of interest, but this is not doable taking into account our computational resources.
\\
\\
* As discussed several times, we should also show - if valid - (the data should be there) something about the convergence properties? In the expected case using a proper AF should allow for a faster convergence? Can be shown using the losses?
\\
\\
* Must not be smooth approximations (what should this be in the context of a linear function?), but it would be intersting to show that functions with a similar LC realy provide similar results!
\\
\\
* Is there any way to learn k? See also above?
}

==> sections/related_old.tex <==
\section{Related Work}
\label{sec:related}

In the following, we first give an overview on activation functions in general and then discuss the problem of fine-grained image classification in more detail.

\subsection{Activation Functions}

Starting from simple thresholding functions, initially, the main focus was on squashing functions such as \func{Sigmoid} and \func{Tanh} \cite{pr:hornik91}. In particular, as following the universal approximation theorem \cite{pr:hornik91} any continuous real-valued function can be arbitrary well approximated by a feed-forward network with one hidden layer if the activation function is continuous, bounded, and monotonically increasing. However, such function are suffering from the vanishing gradient problem \cite{pr:hochreiter98}, in particular if the networks are getting deeper. To overcome this problem, various non-squashing functions were introduced, where in particular \relu \cite{pr:nair10} paved the way for the success for deep learning. As the derivative of positive inputs  of \relu is one, the gradient cannot vanish. On the other hand, all negative values are mapped to zero, resulting in two main problems: (1) There is no information flow for negative values, which is known as dying \relu. (2) The statistical mean of activation value is still larger than zero leading to a bias shift in successive layers. Moreover, all negative values are treated equally, which is not desirable for the FGVC task!

To deal with the dying-\relu-problem \func{Leaky} \relu( \lrelu) \cite{pr:maas13} adds a small negative slope for the negative part. However, the deactivation state is not noise-robust and the function is still suffering from the bias shift. Moreover, several evaluation showed that there are no benefits in terms of classification accuracy. An extension to \lrelu are randomized leaky rectified linear units \func{RReLU}s, which randomly set the slope for the negative part.
Both problems can be resolved by using Exponential Linear Unites (\elu) \cite{pr:clevert15}, which are noise robust in the deactivated state robust to noise and eliminate the bias shift in the succeeding layers by pushing mean activation value towards zero. By returning a bounded exponential value for negative inputs \func{ELU} is saturated at a predefined threshold. The idea was later extended by introducing an self-normalization, \selu \cite{pr:klambauer17}, where it is shown that the proposed self-normalizing network converges towards a normal distribution with zero mean and unit variance. However, also \elu and \selu are bounded, contractive functions, which is not beneficial for the FGVC task. 


To increase the flexibility, adaptive parametric activation functions have been proposed. In contrast to the functions discussed above, these learn parameters  to tune themselves during the training. For instance, 
parametric \relu \cite{pr:he15} define different slopes, however, these are learned from the data and are not set randomly as for \func{RReLU}. Similar,  S-shaped \relu (\func{SReLU}) \cite{pr:jin16} is also an adaptive variation of \relu~with four scalar factors. In this way, there are also several extensions to \elu. Parametric \elu~(\ie, \func{PeLU}) \cite{pr:trottier17}, for instance, evades the vanishing gradient problem and to precisely control the bias shift. Moreover, Multiple Parametric Exponential Linear Units (\func{MPeLU}) \cite{pr:li18a} are proposed to support non-convex shapes as well as to cover the solution space of both the rectified and exponential linear units; which in turn, leads to a better classification performance and preferable convergence properties.


%A typical solution is to multiply the activation function by a fixed parameter; but, it is not still an optimal solution for the situation where the best range of amplitudes for internal hidden neurons may change from one layer to another or even among neurons of the same layer. Thereby, an adaptive parameter can be effective\cite{pr:trentin01}. 



To learn more complex activation function, reinforcement learning \cite{pr:ramachandran18} and genetic programming \cite{pr:basirat19} are applied to create and explore complex search spaces to construct new activation functions. In particular, in \cite{pr:ramachandran18} \swish, a combination of a squashing function and \relu,  was found as solution, which has shown to yield better results on a variety of tasks. Similar results were also obtained by \cite{pr:basirat19}. Recently, a theoretic justification for the design has been given in \cite{pr:hayou18}, showing that \swish propagates information better than \relu. As described above, also for \func{Swish} a parametric version was introduced. Even though the thus obtained function yield good results for CGVC, they are not competitive for FGVC as the small differences between the rather similar classes cannot be modelled very well.

\prmk{Some references are missing? Maybe we should extend this discussion?}


\subsection{Fine-grained visual categorization}

\prmk{This discussion might be shortened and included into the introduction? Then, the RW is just focusion on AF, which would make our story more concise?}\mbrmk{yes}

Recently, the significant success of fine-grained visual categorization (FGVC) heavily relies on advances of Convolutions Neural Networks (CNNs). In general, CNNs improves FGVC either by learning discriminative features \cite{mb:sanchez11,mb:perronnin15} or  part local information is merged into CNNs to represent the deep features of object parts.

Bilinear-CNN  \cite{mb:lin15a}  as a notable approach in fine-grained feature learning, computes second order bilinear features interactions using two symmetric CNNs. However, the approach suffers from curse of dimensionality. For that reason,
\cite{mb:gao15} introduced compact bilinear representations based on kernelized analysis of bilinear pooling. Furthermore, to compact and also preserve the algebraic structure of the bilinear feature maps which are ignored in original approach, \cite{mb:kong17} proposed Low-rank bilinear pooling. As a continues line of researches, \cite{mb:cai17} proposed a higher order integration of hierarchical convolutional activations for FGVC. Later, a kernel form of higher order feature interactions are achieved by \cite{mb:cui17}.
%Concerning  feature learning,
%CNNs features have shown better visual representation than hand-crafted features .On the other hand, CNN approaches mainly show impressive results when they are merged by part localization or attention-based learning.

Part localization deals with locating and discovering subtle appearance differences associated with object parts \cite{mb:kraus14}. Part-based R-CNN by Zhang et al.\cite{mb:zhang14}, applied RCNN to learn both whole-object and part detectors while provides hand-crafted geometric constraints between them. As an extension works, Shaoli Huang \cite{mb:huang16} proposed Part-Stacked CNN that enables to uses much more object parts than Part-based R-CNN. \cite{mb:shi15} proposed a multi-proposal consensus network to predict part locations.  Meanwhile, \cite{mb:lin15b} proposed a valve linkage function that connected part localization, alignment and classification together for each part. However, these methods  only used the big parts. Other unsupervised methods 
could generate multiple object parts, but they are not guaranteed to produce small parts with semantic meanings in particular, for non-structured objects like food. Therefore,  attention models is emerging to detect informative regions which include an important local information \cite{mb:yu18, mb:sun18,mb:jaderberg15,mb:chen18,mb:fu17}. Our work is more related to fine-grained feature learning wherein choosing a proper activation function leads to generate more informative features.


 

==> sections/trash.tex <==
%That is, \lrelu forwards propagated variation better than \relu and even \elu. This property seems to be useful for FGVC. 

%Therefore, the performance of FGVC heavily depends on leaning discriminative features, also taking into account the degree of absence of features.

%The answer is to learn not only the ``presence'' of a feature in the current sample but also the ``degree of its absence''. 

%In fact, in FGVC object categories often share a similar appearance. So, the visual differences are very subtle. Therefore, the performance of FGVC strongly depends on leaning discriminative features. In line with a feature's degree of presence or absence, some activation functions like \relu and \elu discriminate between samples only based on features' degree of presence.

%amples share high similarities. Therefore, we need to increase the discriminative power of each neuron by looking further into the features and their impact on the learning algorithm, but the question is what is left to investigate?

%\mbrmk{Overall, feature presence and absence give us the general picture of activation function \ie if features are totally off. Then, the activation function has a saturated area. This saturated area will change based on the `` off state'' value. For value -1 the shape of AF looks like \elu likewise value 0 for \relu.}
%In addition, We found that using a proper activation function like LReLU with a proper Lipchitz constant increases FGVC's performance. 

% Artificial neurons in DNN receive inputs from features, when a feature is present in the current sample, an activation function assigns $value > 0$ to signal to show how strongly a feature is present. The other way around, feature's absence means a detected feature is not present in the current sample and an activation function assigns $value \leq 0$ as the ``degree of absence'' of that feature.



% Concerning \relu, when a feature is absent, the neuron does not propagate any range of variation, and it is clearly in ``off-stat''; \ie its value is $0$. In the case of \elu, the value $-1$ represents the ``off-state'' or the ``deactivation state'' meaning feature is totally absent. In other words, although \elu provides clear information about features that are absent, it does not convey to what degree a particular feature is absent.


of \swish activation function is computed;
 
 \begin{align}
\label{eq:ex}
 {\frac{d f}{d x}} = \frac{\left(e^{-x}\times(x+1)+1\right)}{(1+ e^{-x})^2 }  
\end{align}

 \begin{align}
\label{eq:3}
 k = \sup|{\frac{d f}{d x}}|= \frac{1}{2} \text{ for } x\leq 0
  \end{align}

The Lipschitz constant for negative part is 0.5. As you can see in  following figure the slope of green line is also 0.5 which is Tangent line of Swish activation function .


%Let $(X,d)$ be a metric space defined on a set $X$ and a metric $d:X \times X \rightarrow R$. Then, a mapping $f:X \rightarrow X$ is a contraction if there exists a constant $k \in [0,1)$ such that 

%\begin{equation}
% d(f(x),f(x')) \leq kd(x,x')
% \label{eq:1} 
%\end{equation}

%\noindent for all $x,x' \in X$. Likewise, for $k>1$,  $f$ is an expanding. If the metric $d$ induces a norm $\lVert . \rVert$, then Eq.~\eqref{eq:1} can be re-written as 



%If there exists a real constant $k\ge0$, then $f$ is a Lipchitz continuous  function and $k$ is referred to as \emph{Lipschitz constant} for function $f$. 
%If $0 \leq k < 1$, $f$ maps a metric space onto itself.




%Please note that rewriting a Lipschitz continuous AF in above form preserves Lipschitz continuity for both $n(x)$ and $p(x)$.

%Having distinguished the pieces of an AF that resides in the first and third quadrants of a Cartesian system, we are now able to discuss how to fine tune feature's degree of presence and absence by tweaking Lipschitz constant of $p(x)$ and $n(x)$, respectively.


% This is not true, thus deleted
%In this way, similar features are getting closer, and dissimilar features are pushed away from each other. 

 \subsection{Lipschitz Constant}
 
 Given the negative part of our \prelu,  then $n(x)=\min(kx, 0)$, $k$ is the Lipschitz constant of $n(x)$. Thus, the contraction of \prelu is defined by the constant $k$.  In fact, to define similarities, contractive mappings are useful because they are less sensitive to variations in feature values and shrink the distance between them. In contrast, expanding mappings amplify changes and increase distances between features of different classes \cite{pr:gordon95}. For FGCV, subtle changes and differences are of relevance. Therefore, \prelu with a proper Lipschitz constant can control the amount of amplification of changes (variations) and also increases distance among inter-class features. Thus, we aim at finding the appropriate contraction level for \prb{\prelu} by looking for an ``optimal'' Lipschitz constant in its negative domain. 
 
 For example, $ReLU(x)=\max(x,0)$ maps the presence of the features via identity with Lipschitz constant $1$, whereas all missing features are mapped to zero with Lipschitz constant $0$ dying all information about feature's absence.
 
 \mbrmk{I think we should not say we set slope manually! based on  might be better to say  we define a slope restricted range for negative part of activation function }, however, we are able to define a meaningful, but not critical range by investigating the function's contraction properties. 

\mbrmk{ it is mentioned in \cite{cohen2019universal}," Intuitively, a Lipschitz function is, to a certain degree, smooth. Small changes in the input will produce measured changes in the output. For example, as we alluded to earlier, all differentiable functions with bounded derivative are Lipschitz continuous. 

Perhaps more importantly, 


I think in FGVC, classes are not well separated and distance (c) between classes are short since differences among them are subtle, So, the Lipschitz constants (c/2) which are found by our experiments are in range (0.05, 0.4)}


% \begin{table*}
%     \begin{subtable}{0.27\textwidth}
%     \resizebox{\textwidth}{!}
%     {
%         \begin{tabular}{lccc}\toprule
%             Dataset & \shortstack{\TahX\\(best slop)} & \shortstack{\TahX\\(slop = 0.7)} &\textbf{\shortstack{PReLU\\(best slop)}}  \\
%             \midrule
%             \midrule
%             Birds 200 & 43.48\% & 43.17\%&\textbf{44.75}\%\\
%             %0.35 slop best
%             \midrule
%             Car & 46.15\% &36.89\%&\textbf{47.16}\%\\
%             %0.20-slop best
%             \midrule
%             iFood & \%& 35.24\%&\textbf{42.94}\%\\
%             %0.35 best-slop
%             \midrule
%             Aircraft & 40.32\% &35.04\% &\textbf{40.72}\%\\
%             %0.35 best-slop
%             \midrule
%             Dogs & 37.47\%&33.30\%& \textbf{37.85}\%\\
%             %0.05 slop best
%             \bottomrule
%         \end{tabular}
%     }
%     \caption{}
%     \end{subtable}%
%     \begin{subtable}{0.40\textwidth}
%     \resizebox{\columnwidth}{!}
%     {%
%         \begin{tabular}{lccccc}\toprule
%             Dataset & ELU &  Swish & ReLU & SeLU &\textbf{L*ReLU}  \\
%             \midrule
%             \midrule
%             Birds 200 & \emph{39.12\%} & 38.89\% & 38.18\% &\% & \textbf{44.75}\%\\
%             %0.35 slop best
%             \midrule
%             Car & 41.86\% & \emph{44.72}\% & 33.08\% & \% &\textbf{47.16}\%\\
%             %0.20-slop best
%             \midrule
%             iFood & 38.12\%&  \emph{41.14\%} & 37.67\% &34.67\%&\textbf{42.94}\%\\
%             %0.35 best-slop
%             \midrule
%             Aircraft & 38.97\%&  \emph{39.63\%} & 38.49\% &\% & \textbf{40.72}\%\\
%             %0.35 best-slop
%             \midrule
%             Dogs & 35.67\% & \emph{37.04\%\emph} &  35.17\% &33.65\%& \textbf{37.85}\%\\
%             %0.05 slop best
%             \bottomrule
%         \end{tabular}
%     }
%     \end{subtable}
%     \caption{This is a large table}
%     \label{tbl:large}
% \end{table*}


==> sections/trash_results.tex <==
\pagebreak


\prmk{How large are the differences between the "best" and the "last" accuracy? To be fair and to allow for reproducibilty the latter one should be shown!}

\begin{table}[!ht]
\centering 
\begin{center}
\begin{tabular}{l|*{6}{c}|r|}\hline	
Activation Functions & Dog & Birds  & Car & Food  \\
\hline
LReLU($\alpha=0.05$) & 37.62\% & 38.57 \% &45.91 \% & 41.04 \%\\ 
\hline
LReLU($\alpha=0.10$) & \textbf{37.63}\% & 41.62\% & 46.00 \% & 41.34\%\\
\hline
LReLU($\alpha=0.15$) & 36.94\% & 42.30\% & 46.15 \% & 41.55\%\\
\hline
LReLU($\alpha=0.20$) & 36.03\% & 43.11\% & 46.00 \% & 42.96\%\\
\hline
LReLU($\alpha=0.25$) & 37.34\% & 44.45\% & 46.27\% & 42.57\%\\
\hline
LReLU($\alpha=0.30$) & 36.82\% & 42.63\% & \textbf{46.97}\% & 43.09\%\\
\hline
LReLU($\alpha=0.35$) & 35.40\% & 42.28\% & 46.42\% & 42.87\%\\
\hline
LReLU($\alpha=0.40$) & 34.49\% & 43.75\% & 44.88\% & 41.63\%\\
\hline
LReLU($\alpha=0.45$) & 34.12\% & 44.06\% & 43.73\% & 41.04\%\\
\hline
LReLU($\alpha=0.50$) & 31.99\% & 43.97\% & 37.98\% & 38.93\%\\
\hline
LReLU($\alpha=0.55$) & 32.12\% & 42.64\% & 38.97\% & 38.28\%\\
\hline
LReLU($\alpha=0.60$) & 29.65\% & 43.82\% & 32.93\% & 35.56\%\\
\hline
LReLU($\alpha=0.65$) & 30.02\% & 43.92\% & 33.13\% & 34.37\%\\
\hline
LReLU($\alpha=0.70$) & 29.79\% & 41.11\% & 29.46 \% & 33.16\%\\
\hline
ReLU                 & 36.37\% & 38.38\% & 36.02\% & 37.53\%\\
\hline
ELU                  & 35.61\% & 38.21\% &41.92 \% &37.69\%\\
\hline
Swish                & 37.13\% & 38.53\% &45.49 \% & 40.78\%\\
\hline
\end{tabular}
\label{table:results-detail} % 
\end{center}
\caption{Results of Fine-grained Dataset Classification}
\end{table}


\prmk{Which information is shown in this plot? Is the standard deviation available for all numbers given in the table? If so this might be shown?}



%boxplotaccuracy
\begin{figure}[!ht]
\centering
\begin{subfigure}{0.5\textwidth}
	\centering
	\includegraphics[width=\textwidth]{results/all_acc_boxplot.png}
	\caption{Boxplot}
	\label{fig:boxplot:a}		
\end{subfigure}
\end{figure}
